Learning Not to Learn in the Presence of Noisy Labels

Learning in the presence of label noise is a challenging yet important task: it is crucial to design models that are robust in the presence of mislabeled datasets. In this paper, we discover that a new class of loss functions called the gambler's loss provides strong robustness to label noise across various levels of corruption. We show that training with this loss function encourages the model to "abstain" from learning on the data points with noisy labels, resulting in a simple and effective method to improve robustness and generalization. In addition, we propose two practical extensions of the method: 1) an analytical early stopping criterion to approximately stop training before the memorization of noisy labels, as well as 2) a heuristic for setting hyperparameters which do not require knowledge of the noise corruption rate. We demonstrate the effectiveness of our method by achieving strong results across three image and text classification tasks as compared to existing baselines.

==> ICML2020_Gambler's Loss Provides Robustness to Label Noise_arxiv (1)/figs/early_stop.tex <==
\begin{figure}[t]
\centering
    \begin{subfigure}[b]{1\linewidth}
        \centering
        \includegraphics[width=0.85\textwidth]{plot/es_mnist.png}
        \vspace{-2mm}
        \caption{MNIST, CNN, $r = 0.80$}
        \label{fig: mnist0.85}
    \end{subfigure}
    %\begin{subfigure}[b]{0.33\textwidth}
    %    \centering
    %    \includegraphics[width=1.01\textwidth]{plot/{1cifar10_0.2_0.95}.png}
    %    \vspace{-3mm}
    %    \caption{CIFAR10, ResNet18, $r = 0.2$}
    %    \label{fig: cifar0.2}
    %\end{subfigure}
    \begin{subfigure}[b]{1\linewidth}
        \centering
        \includegraphics[width=0.85\textwidth]{plot/es_cifar10.png}
        \vspace{-2mm}
        \caption{CIFAR10, ResNet18, $r = 0.85$}
        \label{fig: cifar0.85}
    \end{subfigure}
    \vspace{-8mm}
    \caption{\small{Early stopping results on MNIST and CIFAR10. The horizontal line is the predicted early stopping point based on theorem~\ref{theorem}. We see that our predicted early stopping point corresponds to the observed plateau where the testing accuracy (blue solid line) is at maximum, and right before test accuracy starts to decrease.\vspace{-0mm}}}
    \label{fig:earling stopping}
    \vspace{-3mm}
\end{figure}

==> ICML2020_Gambler's Loss Provides Robustness to Label Noise_arxiv (1)/tables/asym_noise.tex <==
\begin{table}[!tbp]
%\setlength\tabcolsep{2.0pt}
\caption{\small{Robustness of the Gambler's loss to asymetric noise. We set $o=2.0$ for this experiment.}}
\label{tab: assymetric}
\begin{center}
\vspace{-5mm}
\begin{tabular}{l|lll}
%\multirow{2}{*}{\bf Dataset} & \multicolumn{3}{c}{Performance Comparisons} & \multicolumn{2}{c}{Early Stopping Comparisons}\\
% & \textit{nll} loss & Gblers & Gblers + AES\\ 
{\bf Dataset} & \textit{nll} loss  & Gblers & Gblers$_{LAES}$\\ 
\hline
MN pairflip $r=0.3$    &  $71.8\pm 0.5$ & $74.7\pm 0.8$ &$96.3\pm 1.5$\\
MN pairflip $r=0.4$   &  $59.6\pm 1.0$ & $63.0\pm 1.0$&$90.6 \pm 2.0$ \\
MN pairflip $r=0.45$   & $55.2\pm 2.1$ & $60.3\pm 1.0$ & $81.3\pm 5.1$\\
\end{tabular}
\vspace{-4mm}
\end{center}
\end{table}

==> ICML2020_Gambler's Loss Provides Robustness to Label Noise_arxiv (1)/tables/cifar_imdb.tex <==
\begin{table}[!tbp]
%\setlength\tabcolsep{2.0pt}
\caption{{On MNIST, using our method always achieves SOTA performance. On CIFAR-10 (CF10), our method is especially strong when the noise level is extreme ($r\sim 0.7, 0.8, 0.85$), agreeing with our finding in the previous section. (*NA means that the ES stopping point is not reached by the algorithm.)}}
\label{tab: improve co-Teaching}
\begin{center}
\vspace{-3.5mm}
\begin{tabular}{l|lllllll}
\multicolumn{1}{c|}{\bf Dataset}   
& \textit{nll} loss & CT  & Gblrs$_{AES}$\\
\hline
\hline
%CF10 $r=0.2$ & $58.1\pm 0.1$ & $\mathbf{71.0\pm0.6}$ & $68.2\pm 0.0$\\
%CIFAR10 $r=0.2$ & $84.6\pm 0.2$ & $82.3\pm 0.1$ & $\mathbf{85.7 \pm 0.2}$ &\\

CF10 $r=0.5$ & $35.4\pm0.2$ & $\mathbf{65.2\pm 0.2}$  &$60.1\pm 0.2$\\

    CF10 $r=0.6$ &$28.3\pm 0.1$ & $\mathbf{61.1\pm 0.2}$  &  $57.1\pm 0.5$\\

CF10 $r=0.7$ & $20.9\pm 0.4$ & $48.9\pm0.2$ & $\mathbf{50.6
\pm 0.5}$\\

CF10 $r=0.8$ & $15.1\pm 0.5$ & $25.0\pm 0.1$    & $\mathbf{40.7\pm 2.0}$\\

CF10 $r=0.85$ & $13.0\pm 0.5$ & $17.3\pm 0.1$ &  $\mathbf{27.0\pm 2.1}$\\
\hline
IMDB $r=0.1$    & $70.3\pm 0.5$& $80.4 \pm 0.2$ & $74.0\pm 0.3$ \\
IMDB $r=0.15$   & $64.3\pm 0.3$& $79.1 \pm 0.5$ & $69.1\pm 0.2$ \\
IMDB $r=0.2$    & $58.7\pm 0.1$& $78.3 \pm 0.5$ & $65.3\pm 0.7$ \\
IMDB $r=0.25$   & $56.4\pm 0.2$& $76.8 \pm 0.5$ & $62.4\pm 0.4$ \\
IMDB $r=0.3$    & $51.8\pm 0.3$& $75.1 \pm 0.6$ & $53.8\pm 0.3$ \\
%CIFAR100 $r=0.2$   & $34.8\pm 0.4$&  $36.6\pm 0.2$ & $37.1\pm 0.2$ & &  \\
%CIFAR100 $r=0.5$   & $26.2\pm 0.3$& $30.2\pm 0.1$ & $31.0 \pm 0.5$ & & \\
%CIFAR100 $r=0.7$   &  & $23.1\pm 0.4$ & $24.3\pm 0.3$ & $15_7$ & \\ 
%CIFAR100 $r=0.8$   &  & $23.1\pm 0.4$ & $24.3\pm 0.3$ & $15_7$ &
\end{tabular}
\vspace{-8mm}
\end{center}
\end{table}

==> ICML2020_Gambler's Loss Provides Robustness to Label Noise_arxiv (1)/tables/early.tex <==
\begin{table}[!tbp]
%\setlength\tabcolsep{2.0pt}
\vspace{-2mm}
\caption{{Early stopping experiment. The number in parenthesis is the average number of epochs until early stopping. Gambler's loss with early stopping (AES) stops faster and at better accuracy.}}
\vspace{-1.5mm}
\label{tab:earlystopping}
\begin{center}

\begin{tabular}{l|cc}
\hline \hline
{\bf Dataset} & VES & Gamblers AES \\ 
\hline
\hline
MN $r=0.2$      & $95.1\pm 0.4\ (95)$  & $\mathbf{98.8\pm 0.1\ (17)}$ \\
MN $r=0.5$      & $79.7\pm 2.0\ (115)$ & $\mathbf{98.0\pm 0.0\ (18)}$ \\
%MN $r=0.65$     & $58.9\pm 2.5\ (115)$ & $\mathbf{97.2\pm 0.2\ (15)}$\\
MN $r=0.8$      & $21.1\pm 0.1\ (117)$ & $\mathbf{93.5\pm 0.3\ (15)}$\\
MN $r=0.85$     & $15.0\pm 1.1\ (110)$ & $\mathbf{85.2\pm 1.7\ (13)}$\\
\hline
IMDB $r=0.1$    & $71.0\pm 0.5\ (46)$ & $\mathbf{74.0\pm 0.4\ (10)}$\\
%IMDB $r=0.15$   & $67.0\pm 0.3\ (21)$ & $\mathbf{69.1\pm 0.1\ (12)}$\\
IMDB $r=0.2$    & $59.6\pm 0.8\ (8)$  & $\mathbf{65.3\pm 0.7\ (12)}$\\
%IMDB $r=0.25$   & $55.6\pm 0.2\ (8)$  & $\mathbf{62.4\pm 0.4\ (9)}$\\
IMDB $r=0.3$    & $51.1\pm 0.2\ (8)$  & $\mathbf{58.2\pm 0.3\ (12)}$\\

\end{tabular}
\vspace{-2em}
\end{center}
\end{table}

==> ICML2020_Gambler's Loss Provides Robustness to Label Noise_arxiv (1)/tables/gamblers.tex <==
\begin{table*}[!tbp]
%\setlength\tabcolsep{2.0pt}
\caption{{Robustness of the Gambler's loss to noisy labels. We see that simply using gambler's loss on label noise problems improve. For the two categories using early stopping, }}
\label{tab:performance}
\begin{center}
\vspace{-0mm}
\begin{tabular}{l|lllll}
\multirow{1}{*}{\bf Dataset} 
& \textit{nll} loss & Gblers  & CT & CT+  & Gbler$_{AES}$\\ 
\hline
\hline
MN $r=0.2$      & $84.7\pm 0.5$  & $96.7\pm 0.2$ &  $97.2\pm 0.0$ & $97.8\pm0.1$  & $\mathbf{99.0\pm 0.1}$ \\
MN $r=0.5$      & $55.1\pm 3.1$  & $91.2\pm 0.7$&  $93.3\pm 0.1$ & $95.4\pm 0.2$ & $\mathbf{98.4\pm 0.2}$ \\
MN $r=0.65$     & $39.7\pm 2.5$  & $85.9\pm 1.1$&  $92.5 \pm 0.1$& $92.5\pm 0.1$  &   $\mathbf{97.6 \pm 0.3}$ \\
MN $r=0.8$      & $19.1\pm 3.0$  & $76.1\pm 0.3$ & $78.1\pm 0.5$& $67.5\pm0.1$& $\mathbf{95.0 \pm 0.5}$\\
MN $r=0.85$     & $14.5\pm 0.7$  & $71.0\pm 1.4$ &  $60.5\pm 0.2$ & $10.1 \pm 0.0$  &$\mathbf{88.0\pm 1.0}$\\
\hline
\end{tabular}
\vspace{-4mm}
\end{center}
\end{table*}

==> ICML2020_Gambler's Loss Provides Robustness to Label Noise_arxiv (1)/tables/mnist_cifar_imdb.tex <==
\begin{table*}[!tbp]
%\setlength\tabcolsep{2.0pt}
\caption{\small{Robustness of the gambler's loss to noisy labels. We see that simply using gambler's loss on label noise settings improves on $nll$ loss. Furthermore, the scheduled gambler's loss achieves SOTA results as compared to other methods when corruption rate is unknown.}}
\label{tab: gambler-comparison}
\begin{center}
\vspace{-4.5mm}
\begin{tabular}{l|c|cc|ccc}
\hline
\hline
\multirow{2}{*}{\bf Dataset} & \multirow{2}{*}{\textit{nll} loss} & \multicolumn{2}{c|}{\textit{requires corruption rate}} & \multicolumn{3}{c}{\textit{agnostic to corruption rate}} \\ %& \multicolumn{3}{c}{Performance Comparisons} &\\
& & Coteaching+ & Gamblers (AES) & $L_q$ Loss & Gamblers & Gamblers + schedule  \\ 
\hline
\hline
MNIST $r=0.2$  & $95.1 \pm 0.2$ & $88.0\pm 0.1$ & $\mathbf{99.0\pm 0.1}$ & $\mathbf{98.9\pm 0.1}$ & $94.8\pm 0.3$ & $98.7\pm 0.1$ \\

MNIST $r=0.5$  & $74.1\pm 1.0$  & $87.2\pm 0.2$ & $\mathbf{98.4\pm 0.2}$ & $97.8\pm 0.2$ & $80.8\pm 0.5$ & $\mathbf{98.2\pm 0.1}$\\

MNIST $r=0.65$ & $54.5\pm 0.5$  & $86.1\pm 0.2$ & $\mathbf{97.6\pm 0.3}$& $82.5\pm 0.6$ & $66.3\pm 0.6$ & $\mathbf{97.9\pm 0.1}$ \\

MNIST $r=0.8$  & $21.7 \pm 0.6$ & $63.8\pm 0.1$ & $\mathbf{95.0\pm 0.5}$& $39.3\pm 1.3$ & $46.7\pm 0.8$ & $\mathbf{95.0\pm 0.1}$  \\

%MN $r=0.85$ & $16.0\pm 0.4$  & $9.7\pm 0.0$  & $\mathbf{19.6\pm 0.7}$  & $15.0\pm 1.1$ \ (110) &$\mathbf{85.2\pm 1.7 \ (13)}$ \\

\hline

%IMDB $r=0.1$    & $76.1\pm 0.4$ & $77.1\pm 0.4$ & $\mathbf{76.3\pm 0.6}$ \\

IMDB $r=0.15$   & $72.7\pm 0.5$ & $\mathbf{77.6\pm 0.4}$ & $75.4\pm 1.0$ & $74.1\pm 1.0$ & $72.7\pm 0.2$ & $\mathbf{75.0\pm 0.6}$\\

IMDB $r=0.2$    & $69.4\pm 0.7$ & $\mathbf{75.0\pm 0.3}$ & $71.6\pm 2.9$ & $70.8\pm 0.8$ & $69.0\pm 0.7$ & $\mathbf{72.8\pm 0.5}$ \\

IMDB $r=0.25$   & $65.4\pm 0.8$ & $\mathbf{72.3\pm 0.4}$ & $70.5\pm 5.8$ & $68.7\pm 0.7$ & $64.8\pm 0.7$ & $\mathbf{68.9\pm 0.5}$ \\

IMDB $r=0.3$    & $54.6\pm 0.1$ & $\mathbf{67.3\pm 0.3}$ & $54.5\pm 2.3$ & $61.7\pm 0.5$ & $59.8\pm 0.9$ & $\mathbf{62.2\pm 2.2}$ \\

\hline

CIFAR10 $r=0.2$  & $52.7 \pm 0.1$ & $\mathbf{52.2\pm 0.1}$ & $52.1\pm 0.3$ & $52.3\pm 0.4$ & $\mathbf{52.9\pm 0.3}$ & $\mathbf{52.8\pm 0.4}$ \\

CIFAR10 $r=0.5$  & $41.1\pm 0.0$  & $47.4\pm 0.0$ & $\mathbf{48.3\pm 0.4}$ & $46.6\pm 0.3$ & $40.6\pm 0.3$ & $\mathbf{51.9\pm 0.2}$ \\

CIFAR10 $r=0.65$ & $31.8\pm 0.4$  & $42.5\pm 0.1$ & $\mathbf{43.2\pm 0.8}$ & $34.5\pm 0.5$  & $30.8\pm 0.3$ & $\mathbf{45.6\pm 0.3}$ \\

CIFAR10 $r=0.8$  & $10.6 \pm 0.5$ & $9.9\pm 0.0$ & $\mathbf{29.7\pm 1.0}$ & $20.1\pm 0.1$ & $18.1\pm 0.2$ & $\mathbf{25.4\pm 0.7}$  \\

%CIFAR10 $r=0.85$ & $11.7\pm 0.1$  & $10.1\pm 0.0$  & $\mathbf{10.0\pm 0.0}$   \\
\end{tabular}
\vspace{-4mm}
\end{center}
\end{table*}

==> ICML2020_Gambler's Loss Provides Robustness to Label Noise_arxiv (1)/tables/pairflip.tex <==
\begin{table*}[!tbp]
%\setlength\tabcolsep{2.0pt}
\caption{\small{Robustness of the gambler's loss to assymetric noise.}}
\label{tab: assymetric}
\begin{center}
%\vspace{-5mm}
\begin{tabular}{l|c|cccc}
\hline
\hline
{\bf Dataset} & {\textit{nll} loss} %\multicolumn{2}{c|}{\textit{requires corruption rate}} & \multicolumn{3}{c}{\textit{agnostic to corruption rate}} \\ %& \multicolumn{3}{c}{Performance Comparisons} &\\
& Coteaching+  & $L_q$ Loss & Gamblers & Gamblers + schedule  \\ 
\hline
\hline
MNIST $r=0.2$  & $83.8\pm 0.9$ & $87.9\pm 0.2$  & $98.7\pm 0.1$ & $82.9\pm 0.7$ & $\mathbf{98.9\pm 0.1}$ \\

MNIST $r=0.3$  & $72.1\pm 1.0$ & $87.6\pm 0.3$ &  $93.4\pm 0.5$ & $73.0\pm 0.8$ & $\mathbf{98.6\pm 0.1}$\\

MNIST $r=0.45$ & $55.3\pm 0.5$ & $\mathbf{74.5\pm 1.0}$ &  $55.5\pm 1.4$ & $55.0\pm 1.2$ & $\mathbf{72.8\pm 3.0}$ \\

%MN $r=0.85$ & $16.0\pm 0.4$  & $9.7\pm 0.0$  & $\mathbf{19.6\pm 0.7}$  & $15.0\pm 1.1$ \ (110) &$\mathbf{85.2\pm 1.7 \ (13)}$ \\

\hline

CIFAR10 $r=0.2$  & $52.7\pm 0.5$ & $52.2\pm 0.1$  & $50.2\pm 0.3$ & $52.4\pm 0.3$ & $\mathbf{56.4\pm 0.3}$ \\

CIFAR10 $r=0.3$  & $47.7\pm 0.8$ & $49.9\pm 0.1$ &  $46.7\pm 0.3$ & $47.5\pm 0.6$ & $\mathbf{54.8\pm 0.3}$\\

CIFAR10 $r=0.45$ & $34.5\pm 1.0$ & $38.9\pm 0.2$ &  $34.6\pm 0.8$ & $24.6\pm 0.8$ & $\mathbf{46.7\pm 1.0}$ \\

\hline

%IMDB $r=0.1$    & $76.1\pm 0.4$ & $77.1\pm 0.4$ & $\mathbf{76.3\pm 0.6}$ \\

% IMDB $r=0.15$   & $72.7\pm 0.5$ & $\mathbf{77.6\pm 0.4}$ & $75.4\pm 1.0$ & $74.1\pm 1.0$ & $72.7\pm 0.2$ & $\mathbf{75.0\pm 0.6}$\\

% IMDB $r=0.2$    & $69.4\pm 0.7$ & $\mathbf{75.0\pm 0.3}$ & $71.6\pm 2.9$ & $70.8\pm 0.8$ & $69.0\pm 0.7$ & $\mathbf{72.8\pm 0.5}$ \\

% IMDB $r=0.25$   & $65.4\pm 0.8$ & $\mathbf{72.3\pm 0.4}$ & $70.5\pm 5.8$ & $68.7\pm 0.7$ & $64.8\pm 0.7$ & $\mathbf{68.9\pm 0.5}$ \\

% IMDB $r=0.3$    & $54.6\pm 0.1$ & $\mathbf{67.3\pm 0.3}$ & $54.5\pm 2.3$ & $61.7\pm 0.5$ & $59.8\pm 0.9$ & $\mathbf{62.2\pm 2.2}$ \\

% \hline

\end{tabular}
\vspace{-4mm}
\end{center}
\end{table*}

==> tables/asym_noise.tex <==
\begin{table}[!tbp]
%\setlength\tabcolsep{2.0pt}
\caption{\small{Robustness of the Gambler's loss to asymetric noise. We set $o=2.0$ for this experiment.}}
\label{tab: assymetric}
\begin{center}
\vspace{-5mm}
\begin{tabular}{l|lll}
%\multirow{2}{*}{\bf Dataset} & \multicolumn{3}{c}{Performance Comparisons} & \multicolumn{2}{c}{Early Stopping Comparisons}\\
% & \textit{nll} loss & Gblers & Gblers + AES\\ 
{\bf Dataset} & \textit{nll} loss  & Gblers & Gblers$_{LAES}$\\ 
\hline
MN pairflip $r=0.3$    &  $71.8\pm 0.5$ & $74.7\pm 0.8$ &$96.3\pm 1.5$\\
MN pairflip $r=0.4$   &  $59.6\pm 1.0$ & $63.0\pm 1.0$&$90.6 \pm 2.0$ \\
MN pairflip $r=0.45$   & $55.2\pm 2.1$ & $60.3\pm 1.0$ & $81.3\pm 5.1$\\
\end{tabular}
\vspace{-4mm}
\end{center}
\end{table}

==> tables/cifar_imdb.tex <==
\begin{table}[!tbp]
%\setlength\tabcolsep{2.0pt}
\caption{{On MNIST, using our method always achieves SOTA performance. On CIFAR-10 (CF10), our method is especially strong when the noise level is extreme ($r\sim 0.7, 0.8, 0.85$), agreeing with our finding in the previous section. (*NA means that the ES stopping point is not reached by the algorithm.)}}
\label{tab: improve co-Teaching}
\begin{center}
\vspace{-3.5mm}
\begin{tabular}{l|lllllll}
\multicolumn{1}{c|}{\bf Dataset}   
& \textit{nll} loss & CT  & Gblrs$_{AES}$\\
\hline
\hline
%CF10 $r=0.2$ & $58.1\pm 0.1$ & $\mathbf{71.0\pm0.6}$ & $68.2\pm 0.0$\\
%CIFAR10 $r=0.2$ & $84.6\pm 0.2$ & $82.3\pm 0.1$ & $\mathbf{85.7 \pm 0.2}$ &\\

CF10 $r=0.5$ & $35.4\pm0.2$ & $\mathbf{65.2\pm 0.2}$  &$60.1\pm 0.2$\\

    CF10 $r=0.6$ &$28.3\pm 0.1$ & $\mathbf{61.1\pm 0.2}$  &  $57.1\pm 0.5$\\

CF10 $r=0.7$ & $20.9\pm 0.4$ & $48.9\pm0.2$ & $\mathbf{50.6
\pm 0.5}$\\

CF10 $r=0.8$ & $15.1\pm 0.5$ & $25.0\pm 0.1$    & $\mathbf{40.7\pm 2.0}$\\

CF10 $r=0.85$ & $13.0\pm 0.5$ & $17.3\pm 0.1$ &  $\mathbf{27.0\pm 2.1}$\\
\hline
IMDB $r=0.1$    & $70.3\pm 0.5$& $80.4 \pm 0.2$ & $74.0\pm 0.3$ \\
IMDB $r=0.15$   & $64.3\pm 0.3$& $79.1 \pm 0.5$ & $69.1\pm 0.2$ \\
IMDB $r=0.2$    & $58.7\pm 0.1$& $78.3 \pm 0.5$ & $65.3\pm 0.7$ \\
IMDB $r=0.25$   & $56.4\pm 0.2$& $76.8 \pm 0.5$ & $62.4\pm 0.4$ \\
IMDB $r=0.3$    & $51.8\pm 0.3$& $75.1 \pm 0.6$ & $53.8\pm 0.3$ \\
%CIFAR100 $r=0.2$   & $34.8\pm 0.4$&  $36.6\pm 0.2$ & $37.1\pm 0.2$ & &  \\
%CIFAR100 $r=0.5$   & $26.2\pm 0.3$& $30.2\pm 0.1$ & $31.0 \pm 0.5$ & & \\
%CIFAR100 $r=0.7$   &  & $23.1\pm 0.4$ & $24.3\pm 0.3$ & $15_7$ & \\ 
%CIFAR100 $r=0.8$   &  & $23.1\pm 0.4$ & $24.3\pm 0.3$ & $15_7$ &
\end{tabular}
\vspace{-8mm}
\end{center}
\end{table}

==> tables/gamblers.tex <==
\begin{table*}[!tbp]
%\setlength\tabcolsep{2.0pt}
\caption{{Robustness of the Gambler's loss to noisy labels. We see that simply using gambler's loss on label noise problems improve. For the two categories using early stopping, }}
\label{tab:performance}
\begin{center}
\vspace{-0mm}
\begin{tabular}{l|lllll}
\multirow{1}{*}{\bf Dataset} 
& \textit{nll} loss & Gblers  & CT & CT+  & Gbler$_{AES}$\\ 
\hline
\hline
MN $r=0.2$      & $84.7\pm 0.5$  & $96.7\pm 0.2$ &  $97.2\pm 0.0$ & $97.8\pm0.1$  & $\mathbf{99.0\pm 0.1}$ \\
MN $r=0.5$      & $55.1\pm 3.1$  & $91.2\pm 0.7$&  $93.3\pm 0.1$ & $95.4\pm 0.2$ & $\mathbf{98.4\pm 0.2}$ \\
MN $r=0.65$     & $39.7\pm 2.5$  & $85.9\pm 1.1$&  $92.5 \pm 0.1$& $92.5\pm 0.1$  &   $\mathbf{97.6 \pm 0.3}$ \\
MN $r=0.8$      & $19.1\pm 3.0$  & $76.1\pm 0.3$ & $78.1\pm 0.5$& $67.5\pm0.1$& $\mathbf{95.0 \pm 0.5}$\\
MN $r=0.85$     & $14.5\pm 0.7$  & $71.0\pm 1.4$ &  $60.5\pm 0.2$ & $10.1 \pm 0.0$  &$\mathbf{88.0\pm 1.0}$\\
\hline
\end{tabular}
\vspace{-4mm}
\end{center}
\end{table*}
